Unveiling Fiber Networks and Core Formation in the DR21 South Filament

We present high-resolution ($\sim$1000 AU) 3 mm observations with the NOrthern Extended Millimeter Array toward the DR21 South Filament, aiming to reveal its internal fragmentation and search for deeply embedded star-forming activities. Both the continuum and molecular line emissions align well with the filament axis traced by the low-resolution ($\sim$18$^{\prime\prime}$) column density map. The 3 mm continuum, CS (2$-$1), and HCO$^+$ (1$-$0) emissions reveal continuous and diffuse structures with measured FWHM widths of 0.054, 0.029, and 0.030 pc, respectively. In contrast, the H$^{13}$CO$^+$ (1$-$0) emission appears more clumpy and localized. The non-thermal motion in the filament is predominantly subsonic to transonic. We detect 13 dense cores in NH$_2$D (1$_{11}-1_{01}$), three of which coincide with continuum peaks; virial analysis suggests most are gravitationally bound. Using a friend-of-friend algorithm, we identify 32, 34, and 22 velocity-coherent fibers from the CS, HCO$^+$, and H$^{13}$CO$^+$ data, respectively. Compared to fibers traced by CS and HCO$^+$, H$^{13}$CO$^+$ fibers are more frequently associated with NH$_2$D cold cores and exhibit higher average mass-per-unit-length values. Differences among CS, HCO$^+$, and H$^{13}$CO$^+$ emissions likely arise from variations in effective critical densities. These results are consistent with a hierarchical structure, in which the 3.6-pc DR21SF contains velocity-coherent fibers and gravitationally bound dense cores.

==> figs_tabs.tex <==
%-----------------------------------------------------------------------
\begin{table*}
% \centering
\movetableright=-0.3in
\caption{Mach Number}  \label{tab_mach}
\begin{tabular}{c c c ccc ccc}
\hline\hline
Molecules & Pixel & Single & $\mathcal{M}$ & $\mathcal{M}_{\rm mean}$ & $\mathcal{M}_{\rm median}$ & $\mathcal{M}$ $\leq$ 1 & 1 $<$ $\mathcal{M}$ $\leq$ 2 & $\mathcal{M}$ $>$ 2 \\
 & Numbers & Component & & & & & & \\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\
\hline
%\noalign{\smallskip}
CS        & 7740 & 71.0\% & 0.03$-$4.51 & 1.10 & 1.02 & 48.0\% & 47.2\% & 4.8\% \\
HCO$^{+}$ & 5639 & 75.6\% & 0.02$-$5.40 & 1.19 & 1.08 & 42.3\% & 49.5\% & 8.2\% \\
H$^{13}$CO$^{+}$ & 5372 & 78.7\% & 0.05$-$4.66 & 0.98 & 0.97 & 54.9\% & 44.0\% & 1.1\% \\
\hline\hline
\end{tabular}
\end{table*}
%-----------------------------------------------------------------------

%-----------------------------------------------------------------------
\begin{table*}
\centering
\caption{Physical Parameters of the NH$_{2}$D Cores.}  \label{tab_nh2d}
\footnotesize
\begin{tabular}{c cc ccc cc ccc cc}
\hline\hline
CoreID & R.A. & Decl. & Maj $\times$ Min & P.A. & R & $\sigma_{\rm obs}$ & V$_{\rm LSR}$ & S$_{\nu}$ & T$_{\rm dust}$ & M$_{\rm gas}$ & $\alpha_{\rm vir}$ & T$_{\rm vir}$ \\
 & (hh:mm:ss) & (hh:mm:ss) &  &  &  &  &  &  &  &  &  & \\
 & (J2000) & (J2000) & ($^{\prime\prime}$ $\times$ $^{\prime\prime}$) & (deg) & (pc) & (km s$^{-1}$) & (km s$^{-1}$) & (mJy) & (K) & (M$_{\odot}$) &  & (K) \\
\hline
\noalign{\smallskip}
 1  & 20:38:59.247 & 42:17:12.687 & 11.9 $\times$ 4.2 & 78.7  & 0.024 & 0.210 & $-$1.03 & 2.17  & 19.0 & 2.26  & 1.00 & 15 \\
 2  & 20:39:01.415 & 42:17:15.998 &  6.1 $\times$ 3.6 & 111.7 & 0.016 & 0.255 & $-$2.73 & 2.14  & 18.7 & 2.26  & 0.69 & 10 \\
 3  & 20:39:02.156 & 42:16:54.160 &  6.7 $\times$ 4.4 & 45.5  & 0.018 & 0.260 & $-$1.22 & 1.68  & 18.6 & 1.79  & 1.24 & 15 \\
 4  & 20:39:01.662 & 42:16:54.953 &  6.0 $\times$ 5.2 & 90.2  & 0.019 & 0.230 & $-$2.77 & 0.786 & 18.6 & 0.840 & 1.95 & 10 \\
 5  & 20:39:03.648 & 42:16:41.928 &  5.9 $\times$ 4.7 & 44.4  & 0.018 & 0.188 & $-$1.79 & 0.587 & 18.7 & 0.620 & 1.90 & 10 \\
 6  & 20:39:03.215 & 42:16:44.404 &  6.3 $\times$ 4.1 & 24.2  & 0.017 & 0.167 & $-$1.76 & $-$   & $-$  & $-$   & $-$  & $-$ \\ 
 7  & 20:39:06.342 & 42:15:24.181 &  6.3 $\times$ 3.8 & 81.8  & 0.016 & 0.186 & $-$2.10 & 0.596 & 20.5 & 0.568 & 1.89 & 15 \\
 8  & 20:39:12.076 & 42:12:58.027 &  9.0 $\times$ 4.0 & 52.4  & 0.020 & 0.206 & $-$3.47 & 0.389 & 19.5 & 0.392 & 3.87 & 10 \\
 9  & 20:39:11.490 & 42:13:04.312 &  6.4 $\times$ 3.6 & 52.8  & 0.016 & 0.230 & $-$3.23 & $-$   & $-$  & $-$   & $-$  & $-$ \\
 10 & 20:39:11.025 & 42:13:28.114 &  4.8 $\times$ 2.3 & 78.2  & 0.016 & 0.317 & $-$2.91 & $-$   & $-$  & $-$   & $-$  & $-$ \\
 11 & 20:39:15.503 & 42:11:57.030 & 10.4 $\times$ 3.8 & 77.1  & 0.021 & 0.209 & $-$4.06 & 0.431 & 19.5 & 0.435 & 4.57 & 15 \\
 12 & 20:39:15.127 & 42:10:54.980 &  4.5 $\times$ 3.6 & 90.8  & 0.014 & 0.178 & $-$4.84 & $-$   & $-$  & $-$   & $-$  & $-$ \\
 13 & 20:39:16.241 & 42:10:26.514 &  5.2 $\times$ 3.3 & 10.5  & 0.014 & 0.245 & $-$4.94 & $-$   & $-$  & $-$   & $-$  & $-$ \\
\hline\hline
\end{tabular}
\end{table*}
%----------------------------------------------------------------------


%---------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=59mm]{figures/Conti.pdf}
%    \includegraphics[width=59mm]{figures/HCO+_m0.pdf}
%    \includegraphics[width=59mm]{figures/CS_m0.pdf}
%      \caption{Moment-0 maps for continuum HCO+ and cs}
%   \label{fig:m0}
% \end{figure}
% %---------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=88mm]{figures/H13CO+_m0.pdf}
%    \includegraphics[width=88mm]{figures/NH2D_m0.pdf}
%      \caption{Moment-0 maps for h13cop and nh2d}
%   \label{fig:core_m0}
% \end{figure}
% %-----------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=88mm]{figures/hcop_v0.pdf}
%    \includegraphics[width=88mm]{figures/cs_v0.pdf}
%      \caption{Moment-1 maps for HCO+ and cs}
%   \label{fig:m1}
% \end{figure}
% %-----------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
   
%    \includegraphics[width=170mm]{figures/H13CO+_PV.pdf}\\
%    \includegraphics[width=170mm]{figures/HCO+_PV.pdf}\\
%    \includegraphics[width=170mm]{figures/CS_PV.pdf}
%      \caption{PV maps for h13cop HCO+ and cs}
%   \label{fig:pv}
% \end{figure}
% %-----------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=88mm]{figures/conti_fiber.png}
%    \includegraphics[width=88mm]{figures/hcop_fiber.png}\\
%    \includegraphics[width=88mm]{figures/cs_fiber.png}
%    \includegraphics[width=88mm]{figures/fiber.png}
%      \caption{fibers for continuum, HCO+ and cs}
%   \label{fig:filas}
% \end{figure}
% %-----------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=59mm]{figures/conti_width.png}
%    \includegraphics[width=59mm]{figures/hcop_width.png}
%    \includegraphics[width=59mm]{figures/cs_width.png}
%      \caption{fiber widths for continuum h13cop HCO+ and cs}
%   \label{fig:wid}
% \end{figure}
% %-----------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=88mm]{figures/hcop_mach.pdf}
%    \includegraphics[width=88mm]{figures/cs_mach.pdf}
%      \caption{Mach maps for continuum HCO+ and cs}
%   \label{fig:mach}
% \end{figure}
% %-----------------------------------------------------------------------

% %-----------------------------------------------------------------------
% \begin{figure}[h!]
%    \includegraphics[width=44mm]{figures/core1.pdf}
%    \includegraphics[width=44mm]{figures/core2.pdf}
%    \includegraphics[width=44mm]{figures/core3.pdf}
%    \includegraphics[width=44mm]{figures/core3.2.pdf}\\
%    \includegraphics[width=44mm]{figures/core4.pdf}
%    \includegraphics[width=44mm]{figures/core5.pdf}
%    \includegraphics[width=44mm]{figures/core6.pdf}
%    \includegraphics[width=44mm]{figures/core6_1.pdf}\\
%    \includegraphics[width=44mm]{figures/core7.pdf}
%    \includegraphics[width=44mm]{figures/core8.pdf}
%    \includegraphics[width=44mm]{figures/core9.pdf}
%      \caption{nh2d cores}
%   \label{fig:nh2d_cores}
% \end{figure}
% %-----------------------------------------------------------------------


